Velocity Probability Distribution Function in the Crossover and the Viscous Range

We derive a multifractal model for the velocity probability density distribution function (PDF), which is valid from the inertial range to the viscous range. The model gives a continuous evolution of velocity PDFs from large to small scales. It also predicts the asymptotic form of the PDF of velocity gradients. More importantly, the model captures the crossover range behavior and thus allows us to address the transition observed in the Helium turbulence experiment[Tabeling et. al., Phys. Rev. E53, 1613 (1996)] quantitatively. We compare both the PDFs and the structure functions predicted by this model with the experiments from the inertial range to the smallest scale resolved by the experiment. The model also predicts that the flatness measured in the crossover region can decrease with the Reynolds number.

==> pictures/fig-flat-exp.tex <==
% GNUPLOT: LaTeX picture with Postscript
\setlength{\unitlength}{0.1bp}
\special{!
%!PS-Adobe-2.0
%%Creator: gnuplot
%%DocumentFonts: Helvetica
%%BoundingBox: 50 50 770 554
%%Pages: (atend)
%%EndComments
/gnudict 40 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/vshift -33 def
/dl {10 mul} def
/hpt 31.5 def
/vpt 31.5 def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke gnulinewidth 2 mul setlinewidth } def
/AL { stroke gnulinewidth 2 div setlinewidth } def
/PL { stroke gnulinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 dl 2 dl] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 0 1 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 0 1 DL } def
/LT2 { PL [2 dl 3 dl] 1 0 0 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/P { stroke [] 0 setdash
  currentlinewidth 2 div sub M
  0 currentlinewidth V stroke } def
/D { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  P } def
/A { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/B { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  P } def
/C { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/T { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  P  } def
/S { 2 copy A C} def
end
%%EndProlog
}
\begin{picture}(3600,2160)(0,0)
\special{"
%%Page: 1 1
gnudict begin
gsave
50 50 translate
0.100 0.100 scale
0 setgray
/Helvetica findfont 100 scalefont setfont
newpath
-500.000000 -500.000000 translate
LTa
LTb
480 151 M
31 0 V
2906 0 R
-31 0 V
480 478 M
31 0 V
2906 0 R
-31 0 V
480 710 M
31 0 V
2906 0 R
-31 0 V
480 890 M
31 0 V
2906 0 R
-31 0 V
480 1037 M
31 0 V
2906 0 R
-31 0 V
480 1162 M
31 0 V
2906 0 R
-31 0 V
480 1270 M
31 0 V
2906 0 R
-31 0 V
480 1365 M
31 0 V
2906 0 R
-31 0 V
480 1450 M
63 0 V
2874 0 R
-63 0 V
480 2009 M
31 0 V
2906 0 R
-31 0 V
480 151 M
0 63 V
0 1795 R
0 -63 V
775 151 M
0 31 V
0 1827 R
0 -31 V
947 151 M
0 31 V
0 1827 R
0 -31 V
1069 151 M
0 31 V
0 1827 R
0 -31 V
1164 151 M
0 31 V
0 1827 R
0 -31 V
1242 151 M
0 31 V
0 1827 R
0 -31 V
1307 151 M
0 31 V
0 1827 R
0 -31 V
1364 151 M
0 31 V
0 1827 R
0 -31 V
1414 151 M
0 31 V
0 1827 R
0 -31 V
1459 151 M
0 63 V
0 1795 R
0 -63 V
1754 151 M
0 31 V
0 1827 R
0 -31 V
1926 151 M
0 31 V
0 1827 R
0 -31 V
2048 151 M
0 31 V
0 1827 R
0 -31 V
2143 151 M
0 31 V
0 1827 R
0 -31 V
2221 151 M
0 31 V
0 1827 R
0 -31 V
2286 151 M
0 31 V
0 1827 R
0 -31 V
2343 151 M
0 31 V
0 1827 R
0 -31 V
2393 151 M
0 31 V
0 1827 R
0 -31 V
2438 151 M
0 63 V
0 1795 R
0 -63 V
2733 151 M
0 31 V
0 1827 R
0 -31 V
2905 151 M
0 31 V
0 1827 R
0 -31 V
3027 151 M
0 31 V
0 1827 R
0 -31 V
3122 151 M
0 31 V
0 1827 R
0 -31 V
3200 151 M
0 31 V
0 1827 R
0 -31 V
3265 151 M
0 31 V
0 1827 R
0 -31 V
3322 151 M
0 31 V
0 1827 R
0 -31 V
3372 151 M
0 31 V
0 1827 R
0 -31 V
3417 151 M
0 63 V
0 1795 R
0 -63 V
480 151 M
2937 0 V
0 1858 V
-2937 0 V
480 151 L
LT0
3174 1846 D
3219 710 D
2924 809 D
2629 961 D
2335 1156 D
2040 1326 D
1745 1481 D
LT1
3174 1746 A
3185 722 A
2890 791 A
2595 852 A
2301 946 A
2006 1102 A
1711 1102 A
1417 1377 A
LT2
3174 1646 B
3383 673 B
3089 736 B
2794 802 B
2499 887 B
2205 966 B
1910 1035 B
1615 1101 B
1321 1169 B
1026 1198 B
LT3
3174 1546 C
3348 700 C
3053 771 C
2759 842 C
2464 905 C
2169 975 C
1875 1068 C
1580 1192 C
1285 1316 C
990 1376 C
LT4
3174 1446 T
3279 692 T
2984 763 T
2689 839 T
2394 920 T
2100 1007 T
1805 1101 T
1510 1207 T
1216 1284 T
921 1302 T
stroke
grestore
end
showpage
}
\put(3054,1446){\makebox(0,0)[r]{Re=2.88E4}}
\put(3054,1546){\makebox(0,0)[r]{Re=1.17E4}}
\put(3054,1646){\makebox(0,0)[r]{Re=1.07E4}}
\put(3054,1746){\makebox(0,0)[r]{Re=1.86E3}}
\put(3054,1846){\makebox(0,0)[r]{Re=1.36E3}}
\put(1948,2109){\makebox(0,0){Flatness (Experiment)}}
\put(3417,51){\makebox(0,0){1}}
\put(2438,51){\makebox(0,0){0.1}}
\put(1459,51){\makebox(0,0){0.01}}
\put(480,51){\makebox(0,0){0.001}}
\put(420,1450){\makebox(0,0)[r]{10}}
\end{picture}


==> pictures/fig-flattheo.tex <==
% GNUPLOT: LaTeX picture with Postscript
\setlength{\unitlength}{0.1bp}
\special{!
%!PS-Adobe-2.0
%%Creator: gnuplot
%%DocumentFonts: Helvetica
%%BoundingBox: 50 50 770 554
%%Pages: (atend)
%%EndComments
/gnudict 40 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/vshift -33 def
/dl {10 mul} def
/hpt 31.5 def
/vpt 31.5 def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke gnulinewidth 2 mul setlinewidth } def
/AL { stroke gnulinewidth 2 div setlinewidth } def
/PL { stroke gnulinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 dl 2 dl] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 0 1 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 0 1 DL } def
/LT2 { PL [2 dl 3 dl] 1 0 0 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/P { stroke [] 0 setdash
  currentlinewidth 2 div sub M
  0 currentlinewidth V stroke } def
/D { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  P } def
/A { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/B { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  P } def
/C { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/T { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  P  } def
/S { 2 copy A C} def
end
%%EndProlog
}
\begin{picture}(3600,2160)(0,0)
\special{"
%%Page: 1 1
gnudict begin
gsave
50 50 translate
0.100 0.100 scale
0 setgray
/Helvetica findfont 100 scalefont setfont
newpath
-500.000000 -500.000000 translate
LTa
LTb
480 151 M
63 0 V
2874 0 R
-63 0 V
480 431 M
31 0 V
2906 0 R
-31 0 V
480 594 M
31 0 V
2906 0 R
-31 0 V
480 710 M
31 0 V
2906 0 R
-31 0 V
480 800 M
31 0 V
2906 0 R
-31 0 V
480 874 M
31 0 V
2906 0 R
-31 0 V
480 936 M
31 0 V
2906 0 R
-31 0 V
480 990 M
31 0 V
2906 0 R
-31 0 V
480 1037 M
31 0 V
2906 0 R
-31 0 V
480 1080 M
63 0 V
2874 0 R
-63 0 V
480 1360 M
31 0 V
2906 0 R
-31 0 V
480 1523 M
31 0 V
2906 0 R
-31 0 V
480 1639 M
31 0 V
2906 0 R
-31 0 V
480 1729 M
31 0 V
2906 0 R
-31 0 V
480 1803 M
31 0 V
2906 0 R
-31 0 V
480 1865 M
31 0 V
2906 0 R
-31 0 V
480 1919 M
31 0 V
2906 0 R
-31 0 V
480 1966 M
31 0 V
2906 0 R
-31 0 V
480 2009 M
63 0 V
2874 0 R
-63 0 V
480 151 M
0 63 V
0 1795 R
0 -63 V
657 151 M
0 31 V
0 1827 R
0 -31 V
891 151 M
0 31 V
0 1827 R
0 -31 V
1010 151 M
0 31 V
0 1827 R
0 -31 V
1067 151 M
0 63 V
0 1795 R
0 -63 V
1244 151 M
0 31 V
0 1827 R
0 -31 V
1478 151 M
0 31 V
0 1827 R
0 -31 V
1598 151 M
0 31 V
0 1827 R
0 -31 V
1655 151 M
0 63 V
0 1795 R
0 -63 V
1832 151 M
0 31 V
0 1827 R
0 -31 V
2065 151 M
0 31 V
0 1827 R
0 -31 V
2185 151 M
0 31 V
0 1827 R
0 -31 V
2242 151 M
0 63 V
0 1795 R
0 -63 V
2419 151 M
0 31 V
0 1827 R
0 -31 V
2653 151 M
0 31 V
0 1827 R
0 -31 V
2773 151 M
0 31 V
0 1827 R
0 -31 V
2830 151 M
0 63 V
0 1795 R
0 -63 V
3006 151 M
0 31 V
0 1827 R
0 -31 V
3240 151 M
0 31 V
0 1827 R
0 -31 V
3360 151 M
0 31 V
0 1827 R
0 -31 V
3417 151 M
0 63 V
0 1795 R
0 -63 V
480 151 M
2937 0 V
0 1858 V
-2937 0 V
480 151 L
LT0
5299 800 D
3220 696 D
3043 747 D
2866 845 D
2690 1024 D
2513 1195 D
2336 1260 D
2159 1276 D
1982 1282 D
1805 1285 D
1629 1286 D
1452 1287 D
1275 1287 D
1098 1288 D
921 1288 D
745 1288 D
LT1
5299 700 A
3220 692 A
3043 732 A
2866 783 A
2690 874 A
2513 1051 A
2336 1241 A
2159 1325 A
1982 1346 A
1805 1353 A
1629 1356 A
1452 1358 A
1275 1359 A
1098 1360 A
921 1360 A
745 1360 A
LT2
5299 600 B
3220 691 B
3043 728 B
2866 766 B
2690 808 B
2513 874 B
2336 1017 B
2159 1230 B
1982 1378 B
1805 1424 B
1629 1436 B
1452 1441 B
1275 1443 B
1098 1444 B
921 1445 B
745 1445 B
LT3
5299 500 C
3220 691 C
3043 727 C
2866 765 C
2690 805 C
2513 863 C
2336 987 C
2159 1196 C
1982 1368 C
1805 1430 C
1629 1446 C
1452 1451 C
1275 1454 C
1098 1455 C
921 1456 C
745 1457 C
LT4
5299 400 T
3220 691 T
3043 727 T
2866 764 T
2690 802 T
2513 852 T
2336 955 T
2159 1150 T
1982 1348 T
1805 1435 T
1629 1457 T
1452 1464 T
1275 1467 T
1098 1469 T
921 1470 T
745 1471 T
stroke
grestore
end
showpage
}
\put(5179,400){\makebox(0,0)[r]{Re=2.88E4}}
\put(5179,500){\makebox(0,0)[r]{Re=1.17E4}}
\put(5179,600){\makebox(0,0)[r]{Re=1.07E4}}
\put(5179,700){\makebox(0,0)[r]{Re=1.86E3}}
\put(5179,800){\makebox(0,0)[r]{Re=1.36E3}}
\put(1948,2109){\makebox(0,0){Flatness (Theory)}}
\put(3417,51){\makebox(0,0){1}}
\put(2830,51){\makebox(0,0){0.1}}
\put(2242,51){\makebox(0,0){0.01}}
\put(1655,51){\makebox(0,0){0.001}}
\put(1067,51){\makebox(0,0){0.0001}}
\put(480,51){\makebox(0,0){1e-05}}
\put(420,2009){\makebox(0,0)[r]{100}}
\put(420,1080){\makebox(0,0)[r]{10}}
\put(420,151){\makebox(0,0)[r]{1}}
\end{picture}

